An Empirical Analysis of Deep Learning for Cardinality Estimation

We implement and evaluate deep learning for cardinality estimation by studying the accuracy, space and time trade-offs across several architectures. We find that simple deep learning models can learn cardinality estimations across a variety of datasets (reducing the error by 72% - 98% on average compared to PostgreSQL). In addition, we empirically evaluate the impact of injecting cardinality estimates produced by deep learning models into the PostgreSQL optimizer. In many cases, the estimates from these models lead to better query plans across all datasets, reducing the runtimes by up to 49% on select-project-join workloads. As promising as these models are, we also discuss and address some of the challenges of using them in practice.

==> EvalFigure_Snippets/fig_cdf_knee.tex <==
% --------------------------------------------------
%  Begin Figures
% --------------------------------------------------

\begin{figure*}[t]
\centering
\begin{subfigure}{.30\linewidth}
\includegraphics[width=\linewidth]{Figures/im_44_cdf_post.png}%
\label{fig:storage_imdb}
\end{subfigure}
\begin{subfigure}{.30\linewidth}
\includegraphics[width=\linewidth]{Figures/d_13_cdf_post.png}%
\label{fig:storage_dmv}
\centering
\end{subfigure}
\begin{subfigure}{.30\linewidth}
\includegraphics[width=\linewidth]{Figures/t_15_cdf_post.png}%
\label{fig:storage_tpch}
\end{subfigure}\\
\caption{CDF of PostgreSQL absolute errors with storage budget: For each curve, we show the knee, $k$, which defines the split between Easy(PostgreSQL) and Hard(PostgreSQL).}
\label{fig:cdf_knee}
\end{figure*}

% --------------------------------------------------
%  End Figures
% --------------------------------------------------

==> EvalFigure_Snippets/tab_hard_2join_complex.tex <==
\begin{table*}[t]
\scalebox{.9}{
\begin{tabular}{c|l|l|}
\cline{2-3}
\multicolumn{1}{l|}{}       & \multicolumn{2}{c|}{\textbf{Queries with Highest Errors from $2Join$}}                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                                           \\ \cline{2-3} 
\multicolumn{1}{l|}{}       & \textbf{Best NN per Dataset}                                                                                                                                                                                                                                                                                           & \textbf{Best RNN per Dataset}                                                                                                                                                                                                                                                                                           \\ \hline
\multicolumn{1}{|c|}{IMDB}  & \begin{tabular}[c]{@{}l@{}}

(cast\_info,name) where role\_id\textless{}= 10 {[}.7M{]}\\ 
(cast\_info,title) where kind\_id \textless{}= 4 and\textbackslash\\         production\_year \textless{}= 2019 and role\_id \textless{}= 6 {[}.7M{]}\\
(cast\_info,name) where role\_id \textless{}= 11 {[}.6M{]} \\
(cast\_info,name) where role\_id \textless{}= 6 {[}.6M{]} \\
(cast\_info,name) where role\_id \textless{}= 8 {[}.6M{]} \\
(cast\_info,name) where role\_id \textless{}= 9 {[}.6M{]} \\
(cast\_info,name) where role\_id \textless{}= 7 {[}.6M{]} \\
(cast\_info,name) where role\_id \textless{}= 5 {[}.6M{]} \\

\end{tabular} & \begin{tabular}[c]{@{}l@{}}

(cast\_info,name) where role\_id \textless{}= 9 {[}2.1M{]}\\
(cast\_info,name) where role\_id\textless{}= 11 {[}2.1M{]}\\ (cast\_info,role\_type) where role\_id \textless{}= 11 {[}1.9M{]} \\
(cast\_info,role\_type) where role\_id \textless{}= 9 {[}1.8M{]} \\
(cast\_info,role\_type) where role\_id \textless{}= 7 {[}1.3M{]} \\
(cast\_info,name) where role\_id \textless{}= 8 {[}1.2M{]} \\
(cast\_info,role\_type) where role\_id \textless{}= 7 {[}1.1M{]} \\
(cast\_info,title) where kind\_id <= 4,production\_year <= 2019,role\_id<= 6 {[}.9M{]} \\


\end{tabular}                                                                                     \\ \hline
\multicolumn{1}{|c|}{DMV}   & \begin{tabular}[c]{@{}l@{}}

(car,accidents) where year\textless{}= 2004 {[}2.8K{]}\\ 
(accidents,time) where year \textless{}= 2005 and month \textless{}= 9 {[}2.4K{]} \\
(accidents,location) where year \textless{}= 2003 {[}2.1K{]}\\ 
(car,accidents) where year\textless{}= 2005 {[}1.9K{]}\\
(car,accidents) where year\textless{}= 2004 {[}1.6K{]}\\
(car,accidents) where year\textless{}= 2003 {[}1.4K{]}\\
(accidents,time) where year\textless{}= 2003 and month \textless{}= 6 {[}1.1K{]}\\
(car,accidents) where year\textless{}= 2002 {[}1.0K{]}\\

\end{tabular}                                                                & \begin{tabular}[c]{@{}l@{}}

(car,accidents) where year\textless{}= 2004 {[}2.5K{]}\\ 
(accidents,location) where year \textless{}= 2004 {[}2.2K{]}\\ 
(accidents,time) where year \textless{}= 2005 and month \textless{}= 9 {[}1.8K{]} \\
(car,accidents) where year\textless{}= 2005 {[}1.7K{]}\\
(car,accidents) where year\textless{}= 2002 {[}1.6K{]}\\
(accidents,location) where year\textless{}= 2002 {[}1.6K{]}\\
(accidents,time) where year\textless{}= 2003 and month \textless{}= 6 {[}.8K{]}\\
(accidents,time) where year\textless{}= 1983 and month \textless{}= 10 {[}.6K{]}\\

\end{tabular}                                                                         \\ \hline
\multicolumn{1}{|c|}{TPC-H} & \begin{tabular}[c]{@{}l@{}}

(lineitem,orders) l\_linenumber \textless{}= 6 and l\_quantity \textless{}=16 {[}100K{]}\\ 
(lineitem,orders) l\_linenumber \textless{}= 7 and l\_quantity\textless{}= 16 {[}94K{]}\\ 
(lineitem,orders) l\_linenumber \textless{}= 2 and l\_quantity \textless{}= 17 {[}65K{]}\\

(lineitem,orders) l\_linenumber \textless{}= 5 and l\_quantity \textless{}= 35 {[}65K{]}\\
(lineitem,orders) l\_linenumber \textless{}= 6 and l\_quantity \textless{}= 27 {[}45K{]}\\
(lineitem,orders) l\_linenumber \textless{}= 7 and l\_quantity \textless{}= 27 {[}40K{]}\\
(lineitem,orders) l\_linenumber \textless{}= 2 and l\_quantity \textless{}= 23 {[}38K{]}\\
(lineitem,orders) l\_linenumber \textless{}= 7 and l\_quantity \textless{}= 16 {[}38K{]}\\


\end{tabular}   & \begin{tabular}[c]{@{}l@{}}

(lineitem,orders) l\_linenumber \textless{}= 6 and l\_quantity \textless{}= 16 {[}125K{]}\\ 
(lineitem,orders) l\_linenumber \textless{}= 7 and l\_quantity\textless{}= 16 {[}122K{]}\\ 
(lineitem,orders) l\_linenumber \textless{}= 5 and l\_quantity \textless{}= 35 {[}87K{]} \\

(lineitem,orders) l\_linenumber \textless{}= 6 and l\_quantity \textless{}= 38 {[}79K{]}\\
(lineitem,orders) l\_linenumber \textless{}= 7 and l\_quantity \textless{}= 23 {[}78K{]}\\
(lineitem,orders) l\_linenumber \textless{}= 6 and l\_quantity \textless{}= 23 {[}75K{]}\\
(lineitem,orders) l\_linenumber \textless{}= 6 and l\_quantity \textless{}= 22 {[}74K{]}\\
(lineitem,orders) l\_linenumber \textless{}= 7 and l\_quantity \textless{}= 34 {[}73K{]}\\

\end{tabular} \\ \hline
\end{tabular}
}
\caption{The $2Join$ Queries that are Easy(PostgreSQL) and with the highest errors from the NN and RNN Models: For each dataset, we show the top eight queries with the highest absolute errors.}
\label{tab:hard_2join_complex}%
\end{table*}
